A Framework for Real-time Safeguarding the Text Generation of Large Language Model

Large Language Models (LLMs) have significantly advanced natural language processing (NLP) tasks but also pose ethical and societal risks due to their propensity to generate harmful content. Existing methods have limitations, including the need for training specific control models and proactive intervention during text generation, that lead to quality degradation and increased computational overhead. To mitigate those limitations, we propose LLMSafeGuard, a lightweight real-time framework that integrates an external validator into decoding, rejecting unsafe outputs while allowing valid ones. We introduce a similarity-based validation approach, simplifying constraint introduction and eliminating the need for control model training. Additionally, LLMSafeGuard employs a context-wise timing selection strategy, intervening LLMs only when necessary. We evaluate LLMSafeGuard on detoxification and copyright safeguarding, demonstrating its superiority over SOTA baselines. In detoxification, LLMSafeGuard reduces toxic output by at least 38.6\% while preserving linguistic quality. Additionally, its context-wise timing selection cuts inference time by at least 24.2\% without compromising effectiveness.

==> 0-abstract.tex <==
%\sw{TODO: 1) add top-k sampling approach. 2) find a baseline for copy right (\url{https://aclanthology.org/2023.inlg-main.3.pdf#page=12.01).}}

Large Language Models (LLMs) have significantly advanced natural language processing (NLP) tasks but also pose ethical and societal risks due to their propensity to generate harmful content. Existing methods have limitations, including the need for training specific control models and proactive intervention during text generation, that lead to quality degradation and increased computational overhead. To mitigate those limitations, we propose \ourTool, a lightweight real-time framework that integrates an external validator into decoding, rejecting unsafe outputs while allowing valid ones.  We introduce a similarity-based validation approach, simplifying constraint introduction and eliminating the need for control model training. Additionally, \ourTool employs a context-wise timing selection strategy, intervening LLMs only when necessary. We evaluate \ourTool on detoxification and copyright safeguarding, demonstrating its superiority over SOTA baselines. In detoxification, \ourTool reduces toxic output by at least 38.6\% while preserving linguistic quality. Additionally, its context-wise timing selection cuts inference time by at least 24.2\% without compromising effectiveness.

==> 1-introduction.tex <==
\section{Introduction}\label{sec:intro}


Large language models (LLMs) have advanced NLP tasks by generating realistic text~\cite{min2023recent,achiam2023gpt,zhang2023survey}. However, they also exhibit unpredictable harmful behaviors, such as generating toxic content, posing ethical and societal risks~\cite{zhuo2023exploring, liang2022holistic}. This necessitates effective safeguards for LLM-generated text.

Recent approaches to safeguarding LLMs from generating unsafe content, such as toxicity and copyright violations, fall into two main categories: fine-tuning and real-time safeguarding~\cite{zhang2023survey}. Fine-tuning adjusts model parameters to enforce safety constraints~\cite{ziegler2019fine,keskar2019ctrl,qian2022controllable} but is computationally expensive~\cite{qi2023fine}. In contrast, real-time safeguarding manipulates the distribution of each subsequent token during decoding without modifying the LLM by typically using an external control model. This makes real-time methods more lightweight and flexible than fine-tuning.








%Recently, a diverse array of approaches have emerged to safeguard the generation of Large Language Models (LLMs) and to prevent them from generating content that violates safety constraints,  such as toxicity and copyright infringement. These approaches can generally be classified into two main families: fine-tuning and real-time safeguarding~\cite{zhang2023survey}. Fine-tuning involves adjusting either some or all of the parameters of an LLM to produce text that aligns with safety constraints~\cite{ziegler2019fine,keskar2019ctrl,qian2022controllable}. However, fine-tuning requires modifying the entire or a portion of the parameters of existing large language models, leading to computational expenses in real-world application scenarios~\cite{qi2023fine}. Real-time safeguarding, on the other hand, aims to safeguard text generation by manipulating the distribution of tokens during the decoding stage without modifying the original LLMs. In real-time safeguarding, an external control model is typically deployed to modify the distribution of each subsequent token during decoding and guides the LLM to generate text that is more likely to meet safety constraints. Among these two families, real-time approaches show promise for safeguarding, as they are more lightweight and flexible, requiring no modification to existing LLMs, compared to fine-tuning approaches.

However, existing approaches in the real-time family exhibit several limitations. \textbf{Limitation} \circled{1} A dedicated control model must be trained for each safety constraint. For instance, to prevent LLMs from generating sensitive topics (e.g., gender-biased content), specific control models need to be trained to assess the token selections. Moreover, prior approaches tightly couple control models with LLMs, requiring joint training~\cite{kim2022critic,Gedi}, which limits flexibility and increases computational costs when adding new constraints.
\textbf{Limitation} \circled{2} They proactively intervene at each token selection~\cite{kim2022critic,pplm,Gedi} and often deviates from the model's natural output, which degrades text quality. This is evidenced by significantly higher perplexity (PPL) scores - 28.96 and 69.30 for GeDi~\cite{Gedi} and CriticControl~\cite{kim2022critic}, compared to 5.6 for unaltered GPT-2-medium output (see Section~\ref{sec:rq1}). \textbf{Limitation} \circled{3} Intervening at each generation step adds significant overhead. For example, applying GeDi~\cite{Gedi} results in 0.98 seconds to generate 50 tokens on GPT-2-medium, eight times slower than generation without interference (0.12 seconds).


To address the limitations, we propose \ourTool, a lightweight and effective framework that enhances the token selection by integrating a similarity-based external validator. This validator rejects candidates violating safety constraints in real-time, allowing only valid ones to proceed. We use demonstration examples of unsafe content (e.g., toxic text) as anchors to assess candidate similarity. Candidates with high similarity are rejected, while dissimilar ones pass through. This method offers flexibility for new constraints without training an extra control model (to address \circled{1}). Note that demonstration examples can be sourced from user input, existing datasets, or even generated by LLMs~\citep{yoo2021gpt3mix,feng2021survey}. By validating the top candidates during the decoding stage, our approach minimizes the impact on the quality of model output (to address \circled{2}). To avoid step-by-step intervention, we design a strategy that adjusts validation frequency based on candidate similarity to demonstration examples. Validation occurs more frequently when candidates are similar, and less frequently otherwise (to address \circled{2} and \circled{3}).


%We propose a similarity-based validation approach that uses a certain number of provided demonstration examples that violate safety constraints (e.g., toxic text) as the anchor. Specifically, \ourTool assesses the similarity between top candidates and the demonstration examples. Candidates exhibiting high similarity are rejected promptly, while dissimilar ones are deemed valid and will be processed through the beam search. This method offers flexibility for introducing new safety constraints by simply providing a certain number of demonstration examples and avoids the need for training control models (to address \circled{1}). Note that demonstration examples can be sourced from user input, existing datasets, or even generated by LLMs~\citep{yoo2021gpt3mix,feng2021survey}. By validating the top candidates returned by beam search during the decoding state, our approach minimizes the impact on the quality of model output (to address \circled{2}). Furthermore, to avoid intervening at each time step of text generation, we design a novel strategy to select the timing for validation. This strategy measures the similarity between current candidates and demonstration examples, and adjusts the frequency of validation accordingly. The strategy conducts more frequent validation when candidates are similar to demonstration examples, and less frequent validation otherwise (to address \circled{3} and \circled{2}).

To assess the effectiveness of \ourTool, we evaluate it on two tasks: detoxification and copyright safeguard. \ourTool outperforms SOTA baselines in both tasks. For instance, \ourTool reduces the average toxic score of LLM output at least by 38.6\% compared to the best baseline, meanwhile preserving comparable linguistic quality to the naturally generated output. Our context-wise timing selection strategy could reduce 24.2\% inference time, meanwhile maintaining comparable effectiveness as interfering with the LLM every single step. In addition, \ourTool offers tunable parameters to balance the safeguarding effectiveness and inference cost. 


In summary, this paper makes the following contributions:
\begin{itemize}
    \item We propose a novel framework to safeguard the text generation of LLMs in real-time, in which we introduce a similarity-based validation approach and a novel strategy to select the timing for validation to address the limitations of previous SOTA approaches. 
    \item We conducted extensive experiments and show that our framework significantly outperforms all SOTA baselines in two tasks, detoxification and copyright safeguarding. 
    \item We make our dataset and source code public to facilitate future research\footnote{\url{https://anonymous.4open.science/r/realsafeguard-DFD8}}.
\end{itemize}


==> 2-relatedwork.tex <==
\section{Background \& Related work}\label{sec:related}
\subsection{Large language model}

Large language models use transformer models and are trained using massive datasets. Current LLMs such as ChatGPT~\cite{chatgpt}, GPT-4~\cite{achiam2023gpt}, LLaMA~\cite{llama}, and PaLM2~\cite{Palm2} have proven to achieve SOTA performance in various NLP tasks~\cite{Palm2,llama,achiam2023gpt}. Most popular LLMs are decoder-only models. They learn to produce a distribution for the next token in a sequence given past context as input. Given a prompt sequence of tokens, $c_t$ = \{$x_1$, $x_2$, \dots, $x_t$\} where $x_i$ $\in$ $\nu$
and $\nu$ is a vocabulary of tokens, we can produce a distribution $p(X_{t+1}|c_t)$ for the next token in the sequence during the decoding stage following equations below: 
\hspace{-0.1in}
\begin{align}\label{eq:1}
    logit_t &= f_{\theta}(c_t)\\
    p(X_{t+1}|c_t) &= \operatorname{softmax}(logit_t)
\end{align}
,where $logit_t$ is the logit vector given by a LLM $f_{\theta}$. 

% There are two common methods to generate a continuation of the prompt $c_t$ during the decoding. 
% \noindent\textbf{Greedy.} Tokens are generated by iteratively choosing the most likely token from $p(X_{t+1}|c_t)$, and updating the prompt as $c_t$.
% %\xm{maybe three sampling??}

% \noindent\textbf{Beam Search.} In this approach, a set of $2K$ most likely candidates is maintained at each timestep before pruning back down to $K$ at the last step~\cite{meister-etal-2020-best}. For a given candidate at timestep $t$, $b_t$ = \{$b_1$, $b_2$, \dots ,$b_t$\}, the likelihood $l$ is computed as:

% \begin{equation}
% l(b_t) = \sum_{j\leq t} \log p(b_j|b_{<j})
% \end{equation}
% %\xm{ eq 3 should together with eq 2??}
% We modify the beam search process to prevent the output that violates safety constraints during the decoding stage.

\subsection{Safeguarding large language models}\label{sec:relatedWorkSafeguard}
There are three families of approaches to safeguarding large language models based on where and how the safeguard is applied to LLMs. 

% safeguard the output of LLM
The first family focuses on safeguarding the input of LLM, i.e., prompt. The approaches of this family typically apply a safety net on the input of LLMs to detect and filter out prompts that violate safety constraints~\cite{inan2023llama,wu2023defending,xie2024gradsafe}. For instance, Inan et al. developed LlamaGuard~\cite{inan2023llama}, in which they developed a classifier to detect unsafe prompts (e.g., violence and sexual content). %Companies like Microsoft and OpenAI also provide APIs to detect unsafe prompts, e.g., Azure AI Content Safety API~\footnote{https://azure.microsoft.com/en-us/products/ai-services/ai-content-safety} and OpenAI Moderation API~\footnote{https://platform.openai.com/docs/guides/moderation/}. 

The second family fine-tunes existing models to enforce safety constraints in text generation~\cite{ziegler2019fine,qian2022controllable,bai2022constitutional,liu-etal-2020-data,ouyang2022training}. For example, Bai et al. introduced a ``Constitutional AI'' method, employing supervised and reinforcement learning to train a harmless AI which can self-improves and responds to harmful queries though explaining objections without extensive human-labeled data. Qian et al. introduced prefix-tuning to steer generation by modifying only a small set of parameters~\cite{qian2022controllable}. In contrast, \ourTool operates at the decoding stage without altering the model itself during decoding.



%\sw{we can shorten it if we need more space}
%Another family focuses on safeguarding the text generation of LLMs in a real-time manner~\cite{pplm,Gedi,liu2021dexperts,yang-klein-2021-fudge}. The approaches of this family, typically construct an external model to guide LLMs to generate text toward a specific direction by modifying the distribution of subsequent tokens at each time step. Let us use the equation~\ref{eq:1} to illustrate how those approaches work. To guide the text generation toward a specific direction, a distribution $p(a|X_{t+1})$ will be computed by the external model, where $a$ is the constraint, and $X_{t+1}$ is the next token. $p(a|X_{t+1})$ provides the probability of the constraint $a$ conditions on $X_{t+1}$. The modified distribution of next token condition on contraint $a$ is then calculated as $p(X_{t+1}|c_t,a) \propto p(X_{t+1}|c_t)\oplus p(a|X_{t+1})$, where $\oplus$ indicates an specific operation between $p(X_{t+1}|c_t)$ and $p(a|x_{t+1})$. For example, a widely used operation is to multiply them~\cite{kim2022critic,Gedi}. Therefore, the key novelty in the family is to build an effective external model (discriminator) to estimate $p(a|X_{t+1})$. For instance, FUDGE learns a binary predictor for predicting whether a constraint will become true in the complete future, based on an incomplete sequence prefix ($c_t$)~\cite{yang-klein-2021-fudge}. Similarly, CriticControl learns a critic network as the discriminator using Actor-Critic reinforcement learning framework~\cite{kim2022critic}. GeDi~\cite{Gedi} and DExperts~\cite{liu2021dexperts} train both conditional classifier and anti-conditional classifier to provide the probabilities $p(a|X_{t+1})$ and $p(\neg a|X_{t+1})$. The decision made by the external discriminator is calculated as the ratio of disagreement between those two classifiers. However, training a discriminator usually requires a large amount of data and is time-consuming~\cite{kim2022critic,Gedi}. Sometimes the discriminator even has to be trained together with the existing LLM, which increases the coupling between the discriminator and existing LLMs~\cite{kim2022critic}. This limitation reduces the flexibility of applying such techniques in real-world LLM applications. Another limitation is that existing approaches actively intervene in the generation of each subsequent token, thereby adversely impacting the quality of text generated by LLMs. Different from previous approaches, our approach does not need to train an external discriminator to proactively interfere with the distribution of the next tokens. %Instead, we only reject invalid candidates during the beam search and keep the valid ones. Furthermore, we propose a context-wise strategy to avoid interfering with text generation of each time step.


Another family safeguards LLM text generation in real-time by using external models to adjust token distributions at each step~\cite{pplm,Gedi,liu2021dexperts,yang-klein-2021-fudge}. Given a constraint $a$ and next token $X_{t+1}$, these models estimate $p(a|X_{t+1})$ and modify the token distribution as $p(X_{t+1}|c_t,a) \propto p(X_{t+1}|c_t) \oplus p(a|X_{t+1})$, where \( \oplus \) represents a predefined operation ( multiplication)~\cite{kim2022critic,Gedi}. The key novelty in the family is to build an effective external model (discriminator) to estimate $p(a|X_{t+1})$.   
For instance, CriticControl trains a critic network (discriminator) using reinforcement learning~\cite{kim2022critic}. GeDi and DExperts use conditional and anti-conditional classifiers to compute constraint probabilities and guide generation through their ratio~\cite{Gedi, liu2021dexperts}. However, training such discriminators is data-intensive, time-consuming, and often requires co-training with the LLM, increasing coupling and reducing flexibility~\cite{kim2022critic,Gedi}. Unlike these approaches, our method eliminates the need for an external discriminator and does not interfere with token-level distributions frequently.  





==> 3-method.tex <==
\section{Methodology}\label{sec:method}

\begin{figure*}
    \centering
    \includegraphics[width=1\linewidth]{framework.pdf}
    \caption{The workflow of \ourTool involves safeguarding text generation by using an external validator during the decoding stage. Dashed lines signify that validation occurs based on the decision of our context-wise timing selection strategy.}
    \vspace{-0.1in}
    \label{fig:framework}
\vspace{-0.1in}
\end{figure*}

In this section, we introduce our safeguard framework, \ourTool, which integrates an external validator to validate generated candidates. The workflow of \ourTool over time steps is depicted in Figure~\ref{fig:framework}. The top candidates produced during decoding are validated against pre-defined safety constraints using the similarity-based external validator. Invalid candidates are promptly rejected, while valid ones are retained to be sampled for the subsequent time step. To optimize decoding efficiency and prevent excessive interference, we design a context-wise strategy to validate only when necessary.

\begin{algorithm}
\footnotesize
    \caption{Algorithm for \ourTool with top-$k$ sampling.}
    \label{alg:overall}

    \SetKwFunction{rollback}{rollback}
    \SetKwFunction{generatecand}{generatecand}
    \SetKwFunction{}{}
    % \SetKwInput{Input}{Input}
    % \SetKwInput{Output}{Output}
    \SetKwInOut{KwIn}{Input}
    \SetKwInOut{KwOut}{Output}

    \KwIn{Prompt $P$; Top-$k$ searching area $K$; Max token $MT$; Large language model \textbf{$LLM$}; External validator \textbf{$V$}; Threshold for rollback $ThrRB$; Threshold for passing the validation $ThrV$;}
    \KwOut{generated text \textbf{$GT$}}
    %\tcp{initialize the compiler by importing dependent libraries}
    $nextstepForV$, $GT$ = 0, \{\} \\
    \For{$curTS \leftarrow 0$ \KwTo $MT-1$}{

        \If{$curTS$ = $nextstepForV$}{
             $cands$, $invalidCands$, $validCants$ = $GT$,\{\},\{\} \\
            
            %\tcp{Keep sampling until a valid candidate is produced}
            \While{$|validCands| = 0 $}{
                %\tcp{Skip the invalid token when sampling tokens}
                 $nextTokens$ = $LLM$.topKSampling($P$, $K$, $invalidCands[curTS]$) \\
                 $cands$ = $cands \oplus nextTokens$ \\
                 
                $validCands$ = $V$.validate($cands$, $ThrV$) \\
               
                $propInvalid$ = $|cands-validCands|$ / $|cands|$ \\
                %\tcp{Roll back to the previous step if the quality of candidates below a threshold}
                \If{$propInvalid \geq ThrRB$}{
                    $curTS$ = rollback()\\
                    break
                }
                $cands$ = $validCands$ \\
                $invalidCands[curTS]$.append($cands-validCands$)
            }
            $GT$ = randomlySample($cands$) \\
            %\tcp{Decide the next step for validation based on the context information}
            $nextstepForV$ = contextWiseSelection($cands$, $curTS$, $V$) \\
        }\Else{
            $GT$ = $LLM$.topKSampling($P$) \\%\xm{$GT \oplus$ can be removed ?  only $GT$ =  $LLM$.topKSampling($P$)}
        }
        $P$ = $P \oplus GT$  \\
    }
%    $GT$ = $cand$ \\
    \KwRet{$GT$}
    
\end{algorithm}


Algorithm~\ref{alg:overall} demonstrates the detailed procedure of \ourTool with top-$k$ sampling. As discussed in Section~\ref{sec:intro}, validating the output at each time step incurs computational costs and may degrade text quality. To address this, we implement a context-wise strategy (line 18) to select the timing of next validation, which reduces unnecessary interference in the text generation process of LLMs and validation costs (see Section~\ref{sec:contextwise} for more details). If the validation is needed (lines 3-19), the algorithm initiates by sampling the top-$k$ tokens. Within this process, a similarity-based external validator (see Section~\ref{sec:validator} for more details) is employed to assess the validity of the generated candidate (line 8). For instance, in the detoxification task, the validator examines whether the candidates exhibit toxicity. If the generated candidates are deemed invalid, they are rejected, and new tokens are sampled from the token distribution until valid candidates are produced (lines 5-16). To prevent sampling redundant invalid tokens, they are masked during sampling (line 6). In top-$k$ sampling, we then randomly sample one token from the valid candidates for the next round of token generation (line 17). In such a way, we minimize the influence of interference on the output quality as we always aim to output top candidates if they are valid. It is worth noting that LLMs may veer off course, making it challenging to generate valid candidates in the subsequent time steps. To mitigate this, we introduce a \textit{rollback} mechanism, reverting to the previous validating time step when a pre-defined condition is triggered (lines 10-13). Specifically, we measure the proportion of invalid candidates against the total number of candidates. If this proportion exceeds a defined threshold $ThrRB$ (set to 0.5 in our study) a rollback occurs. Note that if rollback is applied, we go back to the last checkpoint and check step by step until the time step that is applied rollback mechanism to avoid the LLM veering off the course again. Our approach could also be easily adjusted to other sampling techniques, such as beam-search and greedy search. See more details about how to adjust to beam-search and greedy search in Appendix~\ref{app:beamsearch}. 

%\xm{Almost right, but I use 0.5 instead of 1, since even checking step by step, we can not guarantee first top k tokens all past the validator. I also modified some thing in Algorithm 1 please review again.}\sw{ok}




\subsection{Similarity-based external validator}\label{sec:validator}
%\sw{this can be significantly cutted.}
%\sw{reviewed until here}

As discussed in Section~\ref{sec:relatedWorkSafeguard}, existing approaches typically rely on trained discriminators for safety constraints, limiting their flexibility for introducing new safety constraints in real-world LLM applications.

To overcome this, we propose a lightweight similarity-based approach for candidate validation, which offers flexibility for introducing new safety constraints by simply providing a certain number of demonstration examples and avoids the need for training discriminator models. Using a set of demonstration examples ($DE$) that violate safety constraints as anchors, we calculate the cosine similarity between candidates ($C$) and $DE$. Candidates with similarity above a defined threshold ($ThrV$) are rejected. This approach is more flexible than discriminator-based methods, as demonstration examples can be sourced from user input, existing datasets, or generated by LLMs. In our detoxification task, we use examples from an existing dataset (see Section~\ref{sec:task}). For each candidate ($c_i$), we compute the similarity and reject it if it exceeds $ThrV$. Note that reducing $ThrV$ typically enhances the control by \ourTool but adversely impacts both the inference time and the linguistic quality of the output from LLMs.


%As discussed in Section~\ref{sec:relatedWorkSafeguard}, existing approaches typically rely on a discriminator (i.e., a classification model) that requires training for defined safety constraints. This restricts the flexibility of applying those approaches in real-world LLM applications. To address the limitation, we propose a lightweight yet effective similarity-based approach to validate the candidates ($C$). We use a set of demonstration examples ($DE$) that violate the safety constraints as the anchor. We calculate the similarity between the candidates and demonstration examples for validation. Candidates that are similar to $DE$ are deemed invalid and rejected. Consequently, the validation process transforms into providing a set of demonstration examples and calculating their similarity. It is noteworthy that, in real-world applications, demonstration examples could be sourced from user input, existing datasets, or even generated by LLMs. For example, in our detoxification task study, we gather demonstration examples from an existing dataset (refer to Section~\ref{sec:task}). Compared to existing approaches relying on trained discriminators, our validation approach is more flexible and lightweight. Given a list of candidates ($C$) and demonstration examples, for each candidate ($c_i$), we compute the similarity between them using cosine similarity~\cite{singhal2001modern}. If any demonstration example exhibits similarity to a candidate, i.e., surpassing the defined threshold $ThrV$, we deem the candidate invalid. See more details in Appendix~\ref{appedix:validator}. In this study, we empirically set $ThrV$ to 0.3 (see Appendix~\ref{sec:hyperparameters} for more details on the impact of $ThrV$). We employ Sentence-BERT~\cite{reimers2019sentence} to embed $c_i$ and $DE$ for similarity calculation. %\xm{we should think about model output not just only thinks $C^T$, for example  if t = 5  we need to consider about validated sentence combine with $C^t$ 5 to inference KD}.



%Note  that the time complexity of our validation algorithm is $O(|C||DE|)$. If the size of $DE$ is large, the computation time of our algorithm increases linearly. To mitigate this, while still preserving the effectiveness of our algorithm, we propose using a clustering algorithm for data sampling to reduce the size of $DE$ while maintaining the diversity of $DE$ (lines 3-7). Initially, we perform clustering on all $DE$. Subsequently, we randomly select a proportion of $R$ examples from each cluster as our final $DE$. We choose the non-parametric clustering algorithm Mean Shift~\cite{cheng1995mean}, which does not require the user to specify the number of clusters in advance. However, alternative clustering algorithms are also applicable. The clustering algorithm necessitates a metric for measuring the distance between examples. Similar to Algorithm~\ref{alg:validation}, we utilize Sentence-BERT for embedding and cosine similarity for distance measurement. In theory, the effectiveness of our algorithm is proportional to the size of demonstration examples. Practitioners can determine $R$ based on the context of their application (e.g., the trade-off between efficiency and effectiveness). Refer to Section~\ref{sec:rq3} for further insights into the impact of $R$ on \ourTool.





\subsection{\contextwise}\label{sec:contextwise}



\begin{figure}

    \centering
    \subfigure[]{\includegraphics[width=0.235\textwidth]{invalid_candidates_proportion_ticks_interval_5_fontsize_24.pdf}}
    \subfigure[]{\includegraphics[width=0.235\textwidth]{similarity.pdf}}
    \vspace{-0.2in}
    \caption{The proportion of invalid candidates against each time step (a) and the boxplot of similarity between candidates and demonstration examples over each time step (b). }
    \label{fig:invalideProp}
\vspace{-0.2in}
\end{figure}




%\sw{revisit, mention we would like to trade-off between effectiveness and efficiency}
%Intuitively, validating the candidates for each step achieves the strongest control on the output of LLM. However, nothing is free. Such a validation strategy sacrifices efficiency and is computationally expensive. In addition, interfering with the distribution of tokens at each time step negatively affects the linguistic quality of LLMs. To address those, we propose a simple yet effective strategy \contextwise, which allows \ourTool to skip certain steps to avoid over-interference based on the context, i.e., the similarity between the current candidates ($C$) and demonstration examples ($DE$). The design of \contextwise is based on a key observation we made. Figure~\ref{fig:invalideProp} shows the proportion of invalid candidates in each time step in the detoxification task (e.g., protecting from generating toxic content) after applying our validation algorithm while without \contextwise. As we can see, the proportion of invalid candidates generated by LLM declines drastically from 0.42 at the first step to 0.05 after 20 steps' safeguard.\sw{Ximing, let's show the similarity over time as well.} Meanwhile, we also observe a similar trend for the similarity between $C$ and $DE$. We observe a positive correlation between the similarity and proportion of invalid candidates. Our observation suggests that when the similarity between $C$ and $DE$ declines, the likelihood of generating invalid candidates also declines. Therefore, it is not necessary to interfere with the LLM for each single time step, typically after the first several steps' safeguard, the similarity between $C$ and $DE$ is low and the likelihood of generating text that violates safety constraints has been significantly declined.

Validating candidates at each step ensures robust control over LLM outputs but sacrifices efficiency and increases computational costs. Additionally, frequent interference in token distribution may degrade linguistic quality. To mitigate these issues, we propose \contextwise (\textit{\contextwiseAbb}), a novel strategy that allows \ourTool to adaptively determine validation timing based on the similarity between current candidates ($C$) and demonstration examples ($DE$), minimizing unnecessary interference.

The design of \contextwiseAbb stems from a key observation we made. Figure~\ref{fig:invalideProp} (a) illustrates the proportion of invalid candidates at each time step in the detoxification task with our validation algorithm (without \contextwiseAbb). We observe a significant decrease in the proportion of invalid candidates, from 0.42 at the initial step to 0.05 after 25 steps. Additionally, we note a similar trend in the similarity between $C$ and $DE$ (Figure~\ref{fig:invalideProp} (b)).
This suggests that as the similarity decreases, the likelihood of generating invalid candidates diminishes and the model becomes more likely to generate valid output. Consequently, continuous interference at each time step is unnecessary, typically, after the initial safeguarding steps.


Drawing from this observation, we craft \contextwiseAbb to operate in a manner where the candidates $C$ are validated based on their similarity to $DE$. It is designed to balance validation efficiency and effectiveness by dynamically adjusting the validation frequency based on similarity to known unsafe examples. When $C$ closely resembles $DE$, indicating a higher likelihood of constraint violation, we conduct validation more frequently (i.e., the smaller interval between two steps), otherwise we skip larger steps. We formalize this with the equation:

\begin{equation}\label{eq:contextwise}
\scriptstyle
\hspace{-0.3in}
nextStep = curStep + \ceil{2^{\lambda(ThrV - min(similarity(C,DE))}}
\end{equation}
, where $curStep$ is the current step, $nextStep$ is the next validation step, and $\ceil{}$ denotes the ceiling function. The function $similarity(C,DE)$ computes the similarity between each candidate and demonstration pair. Given a validation threshold $ThrV$, high similarity triggers frequent validation (e.g., every step). The specific formula in Equation (3) is motivated by the need to increase step size when the risk of constraint violation is high while reducing unnecessary checks when the risk is low. The use of 2$^{[]}$ ensures that when the similarity to unsafe examples is low, the step size grows exponentially, reducing the frequency of validation. The parameter $\lambda$ controls validation intensity: a higher $\lambda$ skips more steps (less frequent validation), while a lower $\lambda$ ensures stricter oversight. 

%In this study, we empirically set $\lambda$ to 200 (see Section~\ref{sec:hyperparameters_short} for details on its impact).









==> 4-experimental-setting.tex <==
\section{Experimental Setting}\label{sec:experimentalsetting}

% \subsection{Research Questions}
% We evaluate \ourTool in different aspects to answer the following research questions.

% \begin{itemize}
%     \item\rqone
%     \hfill
%     \item \rqtwo
%     \hfill
%     \item \rqthree
% \end{itemize}

% In RQ1, we aim to evaluate the effectiveness of \ourTool in two tasks detoxification and copyright safeguard. In RQ2, we investigate the effectiveness of our \contextwise and its contribution to \ourTool. In RQ3, we investigate the impact of parameters on the effectiveness of \ourTool.



\subsection{Tasks}\label{sec:task}
In this study, we evaluate \ourTool on two tasks detoxification and copyright. Below, we introduce the dataset, evaluation metrics, and baselines for each task.

\subsubsection{Detoxification}

\noindent\textbf{Dataset} We use Jigsaw Toxic Dataset~\footnote{\url{https://kaggle.com/competitions/jigsaw-toxic-comment-classification-challenge}}~\cite{jigsaw-toxic-comment-classification-challenge} for this task by following previous studies~\cite{Gedi,pplm,kim2022critic,qian2022controllable}. We follow the same experimental setting as the previous study~\cite{qian2022controllable}. We use the testing prompts for our evaluation. We selected the toxic samples (toxic score $>$ 0.5) in training data as demonstration examples for our approach.


\noindent\textbf{Evaluation Metrics} We use \textbf{Toxic score (Toxic)} as the evaluation metric by following previous studies~\cite{qian2022controllable,kim2022critic}. Toxic score is a widely used metric to measure the probability of a piece of text being toxic. We use the API provided by Perspective API~\footnote{\url{https://www.perspectiveapi.com/}}, which is a widely used service, to measure the toxic score. Besides the above-mentioned task-specific evaluation metrics, we also deploy the following metrics for both tasks: \textbf{Perplexity (PPL)} Perplexity is a widely-used metric to measure the linguistic quality of text generated by language models~\cite{chen1998evaluation,qian2022controllable,kim2022critic}. In this study, we use API provided by HuggingFace~\footnote{\url{https://huggingface.co/docs/transformers/en/perplexity}} to measure the quality of text generated by LLM. \textbf{Inference time (Time)} Total time required to complete text generation for a given prompt. 


\noindent\textbf{Baselines} We compare \ourTool with the following baselines:
\textbf{\Basemodel} original base model without applying any safeguard techniques. 
\textbf{\Basemodelprompt} Different from \Basemodel, we prepend each prompt with the safeguard sentence ``Generate a non-toxic comment'' by following previous study~\cite{qian2022controllable}. 
We also select two SOTA real-time safeguard approaches as our baselines.
\textbf{Gedi~\cite{Gedi}} is a real-time safeguarding approach, which trains conditional LMs and uses them as discriminators to guide the generation of an LLM, introducing an additional 345M parameters.
\textbf{CriticControl~\cite{kim2022critic}} is a real-time safeguarding approach, guiding token generation from an LLM in the decoding stage with the critic network learned by using reinforcement learning. \textbf{\ourToolClassifier} To demonstrate the effectiveness of our similarity-based validator, we also include a variant of \ourTool in which we replace our similarity-based validator with a toxic classifier. 
\textbf{ContrastivePrefix~\cite{qian2022controllable}} is a fine-tuning approach, which leverages prefix-tuning to train a prefix (a set of small continuous attribute-specific vectors) to guide the generation of LLM. 
%we could replace this with if needed https://github.com/tqzhong/Air-Decoding



\subsubsection{Copyright}
%Large language models may memorize more than just facts, including entire chunks of texts seen during training, and cause copyright violation~\cite{karamolegkoucopyright}. We aim to investigate the effectiveness of \ourTool in safeguarding LLMs from copyright issues, i.e., reducing the risk of LLM generating copyrighted text. To do this,
We use the dataset from previous study~\cite{karamolegkoucopyright}, which is a collection of popular books (e.g., Harry Potter and Lolita). We follow its experimental setting and chunk the books into paragraphs. We then randomly sample 100 paragraphs as our evaluation data. We used the first 50 tokens as the prefix prompt and asked the LLM to continue the generation. We set the max token to 200. For the external validator, we use the chunked paragraphs of all collected books as our demonstration examples.

\noindent\textbf{Evaluation metrics} The copyright status of LLM-generated text is not defined and it is still an open question how to measure the copyright infringement~\footnote{\url{https://en.wikipedia.org/wiki/Wikipedia:Large_language_models_and_copyrigt}}. Therefore, we use \textbf{Longest Common Subsequence (\textbf{LCS})} to evaluate the effectiveness of \ourTool by following previous studies~\cite{karamolegkoucopyright,liang2022holistic}. %LCS is a commonly used metric to measure the repetition of two pieces of text. A larger LCS suggests that two pieces of text are more likely to be the same and violate copyright. 
To reduce the bias from longer completions,  we also calculate the normalized LCS (i.e., \textbf{LCS$_{norm}$}), which is normalized by the length of the completion. Similar to detoxification, we also measure \textbf{PPL} and \textbf{Inference time}.
    
%s\item \textbf{Edit Distance (\textbf{Edit}) \sw{what distance we are using?}} Similarly, we select edit distance by following previous studies~\cite{karamolegkoucopyright,liang2022holistic}. A smaller edit distance indicates that two pieces of text are more similar and more likely to be copyrighted. Similar to LCS, we also compute the normalized edit distance \textbf{Edit$_{norm}$}.




\noindent\textbf{Baselines} We compare \ourTool with the following baselines:
\textbf{\Basemodel} original base model without any interference in the decoding stage. \textbf{\Basemodelprompt} Different from \Basemodel, we prepend each prompt with the safeguarding sentence ``Do not plagiarize the original text''. 
\textbf{Memorization-free Decoding~\cite{ippolito2022preventing}} filters out the tokens that could lead to exact n-grams found in the training data during the decoding stage.

%\subsection{Samplings}
%We evaluate \ourTool on Top-K and Beam Search. 

\subsection{Base large language models and sampling techniques}
For detoxification, we select GPT-2-medium as our base model by following previous studies~\cite{Gedi,pplm,kim2022critic,qian2022controllable}. We also select a more recent model Qwen2.5-7B~\cite{qwen2.5}.
For copyright safeguard, we use LLaMA2-13B and Qwen2.5-7B as our base model since previous studies show that large-sized models are more likely to memorize information from training data and violate copyright~\cite{karamolegkoucopyright,liang2022holistic}. We evaluate \ourTool on two decoding sampling techniques, top-$k$ and beam-search. \textbf{Note that for all baselines, we use top-$k$ sampling by following their default settings.}

We set $ThrV$ and $\lambda$ to 0.3 and 100 in our experiment, respectively. See Section~\ref{sec:hyperparameters} for further details on its impact.

% \subsection{Implementation details}
% %Experiments were conducted on a machine equipped with four Nvidia GeForce GTX 1080 GPUs, a 24-core CPU, and 24 GB of RAM. 
% We begin by downloading the official checkpoints for all evaluated models from HuggingFace. We use the default 32-bit precision mode for GPT2~\cite{huggingfaceOpenAI}. To run LLaMA-13b in our GPU, we use 4-bit precision mode for LLaMA-13b~\cite{huggingface-meta-llama}. The Torch and Transformers packages are employed to perform all the experiments. All experiments are done in Python 3.10. We use Qdrant~\cite{qdrant} as the external knowledge base for storing and retrieving the demonstration examples. we use all-MiniLM-L6-v2~\cite{all-MiniLM-L6-v2} from sentence-transformers as the implementation of Sentence-BERT used in our external validator. %The implemented code and dataset have been made public\footnote{https://anonymous.4open.science/r/realsafeguard-DFD8}.  





%\subsubsection{Approach of RQ3}
%In \ourTool, we have multiple parameters that may impact the effectiveness of \ourTool. $\lambda$ is a threshold in \contextwiseAbb, which is used to determine the intensity of the control of \ourTool. $ThrV$ is a threshold in the validator to determine whether a candidate is valid or not. $R$ is a parameter to determine the proportion of demonstration examples that will be used in the validator. In this RQ, we aim to investigate the impact of those three parameters on the effectiveness of \ourTool. We use the same setting as RQ1 except for the investigated parameters. 



==> 5-results.tex <==
\section{Results}\label{sec:results}
\input{rq1}

\input{rq2}

\input{latex/rq3_short}

==> conclusion.tex <==
\section{Conclusion}\label{sec:conclusion}
In this paper, we propose \ourTool, a lightweight post-processing framework designed to safeguard LLM text generation. Specifically, we introduce a similarity-based validation approach, simplifying constraint introduction and eliminating the need for control model training. Additionally, we introduce a context-wise timing selection strategy, validating the text generation only when necessary. We evaluate \ourTool on two tasks, detoxification, and copyright, demonstrating superior performance compared to baselines. For instance, \ourTool reduces the average toxic score of LLM output by 38.6\% while maintaining linguistic quality for the detoxification task. Moreover, \contextwiseAbb reduces inference time by 24.2\% while maintaining comparable effectiveness as validating each single step. \ourTool provides tunable parameters to balance effectiveness and efficiency.

==> discussion.tex <==
\section{Discussion}\label{sec:dis}

\noindent\textbf{Robustness to noise in demonstration examples}
To evaluate the robustness of our approach to noise in demonstration examples, we conducted experiments on the detoxification task using Qwen-2.5-7B. We introduced varying levels of noise by manually injecting non-toxic examples into the demonstration set. These non-toxic sentences were generated by prompting GPT-3.5 to produce random, innocuous content.
As shown in Table~\ref{tab:noiseimpact}, the presence of noise has minimal impact on the effectiveness of our method. This robustness can be attributed to our similarity-based validation mechanism, which consistently blocks toxic outputs, even when the demonstration set contains irrelevant (non-toxic) examples. In contrast to control model-based approaches trained on noisy data, where the presence of noise may compromise the model’s ability to detect and filter toxic content—our validation mechanism ensures reliable filtering by relying on the core toxic examples. %Regarding diversity, we acknowledge that our approach's effectiveness relies on the diversity of demonstration examples. However, this requirement is not unique to our method; control model-based approaches similarly depend on diverse training data to perform well.

\begin{table}
    \centering
    \scriptsize
    \caption{Impact of noise in demonstration examples.}
    \label{tab:noiseimpact}
    \vspace{-0.1in}
    \begin{tabular}{l|lll}
    \hline
     Noise Level &	Toxic	& PPL	& Time (s)\\
     \hline
     0\%	& 0.027 &	11.27	& 2.34 \\
     %\hline
    10\%	& 0.023 & 	11.88	& 2.35 \\
    %\hline
    30\%	& 0.029	& 11.71	& 2.32 \\
    %\hline
    50\%	& 0.030	& 12.30	& 2.39 \\
    \hline
    \end{tabular}
\vspace{-0.2in}
\end{table}





%\textbf{Guiding LLMs to Generate Context-Aligned Content Under Constraints} This research demonstrates \ourTool's effectiveness in preventing invalid content generation. By leveraging an external knowledge base of unsafe examples, \ourTool validates and filters candidates during decoding. Beyond safeguarding, it can also be adapted to enforce specific constraints, such as steering generation toward a desired topic by selectively approving relevant candidates during beam search.

%\textbf{Real-time hallucination protection.}  Hallucination remains a major challenge for LLMs, as they often generate false information with high confidence~\cite{hallucination2023,zhang2023sirens}. Retrieval Augmented Generation (RAG) helps mitigate this by retrieving relevant information and incorporating it into prompts or validating outputs~\cite{zhang2023sirens,huang2023survey}. However, no existing approach provides real-time hallucination protection during decoding. Our framework can address this gap by validating candidate outputs against facts retrieved from an external knowledge base in real-time, ensuring that generated content aligns with factual information.

%\textbf{Adapting \contextwiseAbb to other real-time safeguarding techniques.} We demonstrate the effectiveness of \contextwiseAbb in selecting the timing for validation based on the context. It is worth noting that \contextwiseAbb is not only applicable to our framework but it could also be applied to other safeguarding techniques, which need to manipulate the token distribution in the decoding stage, such as the real-time safeguarding techniques we introduced in Section~\ref{sec:related}.




==> latex/rq1.tex <==
\subsection{Effectiveness of \ourTool}\label{sec:rq1}
\definecolor{lightgreen}{RGB}{144,238,144} 


%\sw{can we replace contrastivePrefix with \url{https://github.com/tqzhong/Air-Decoding}}, which provide code. otherwise we have to remove it. we cannot say they don't provide code.}

\begin{table}[]
\centering
\caption{Comparison of \ourTool with baselines.}\label{tab:rq1detoxification}
\vspace{-0.1in}
\resizebox{0.5\textwidth}{!}{
\begin{tabular}{l|lll|lll}
\toprule

                \multicolumn{7}{c}{\textbf{Detoxification}}                                                                                                                        \\
\hline
& \multicolumn{3}{c}{\textbf{GPT-2}}      &\multicolumn{3}{|c}{\textbf{Qwen2.5-7B}}                                                                                                             \\

\hline
\textbf{Approach}  &\textbf{Toxic}  & \textbf{PPL}& \textbf{Time} &\textbf{Toxic}  & \textbf{PPL}& \textbf{Time} \\ 
\hline
\textbf{\Basemodel}            & 0.788     & 5.60                  & 0.120         & 0.478	& 8.07	& 1.25         \\ 
\textbf{\Basemodelprompt}  &0.785  & 6.87                    & 0.141       & 0.374	& 8.34	& 1.35             \\ 
\textbf{\ContrastivePrefix}\tablefootnote{We did not find the implementation. We copied the results reported in their paper on GPT-2.}   & 0.176      & 100.18                   & 0.144    &  N/A    &         N/A          &   N/A           \\ 
\textbf{\CriticControl}     & 0.428       & 69.30                   & 0.918     & 0.350	& 50.87	& 4.01          \\ 
\textbf{\Gedi}           & 0.393           & 28.96                    & 0.982    & 0.198	& 25.75	& 3.07               \\ 

%\textbf{\ourToolBS}  & 0.124   & 7.85                  & 0.510                \\ 
\textbf{\ourToolClassifier}   & 0.271      & 17.39                   &1.541     &  0.052    &   12.79                &  2.87            \\ 
\rowcolor{lightgreen}
\textbf{\ourToolTopK}  &0.108 &10.77               & 0.495         & 0.027	& 11.27	& 2.34       \\ 
\rowcolor{lightgreen}
\textbf{\ourToolBS}  &0.124 &7.85               & 0.510           & 0.033	& 9.81	&2.33    \\
\midrule
 \multicolumn{7}{c}{\textbf{Copyright}}              \\

\hline
& \multicolumn{3}{c|}{\textbf{LLaMA2-13B}}      &\multicolumn{3}{|c}{\textbf{Qwen2.5-7B}}                                                                                                             \\

\hline
 \textbf{Approach}        & \textbf{LCS($_{norm}$)} & \textbf{PPL} & \textbf{Time} & \textbf{LCS($_{norm}$)} & \textbf{PPL} & \textbf{Time}\\
 \hline
        \textbf{\Basemodel} & 11.09(0.055) & 2.31 &  17.6 & 8.17(0.054)	& 4.37	& 20.4 \\
          \textbf{\Basemodelprompt} & 10.08(0.050) & 2.67 & 17.9 & 3.87(0.036)	& 4.85	& 20.7 \\
         \textbf{Memorization-free}   &1.28(0.008) & 5.01 & 27.5 & 0.273(0.005)	& 8.56	& 29.8 \\
         \rowcolor{lightgreen}
         \textbf{\ourToolTopK}  &1.08(0.007) & 5.65 &27.2 & 0.137(0.003)	& 8.34	& 29.5 \\
         \rowcolor{lightgreen}
         \textbf{\ourToolBS}  &4.03(0.02) & 3.95 &26.3 & 0.333(0.009) &	7.99	& 29.7
 \\
         \bottomrule
\end{tabular}
}
\vspace{-0.2in}
\end{table}

%\xm{or7.85?}\sw{we are presenting the results of top-k, avoid mixing them}
Table~\ref{tab:rq1detoxification} illustrates the results of \ourTool and the baselines. When applying \ourTool on top-$k$ sampling, \ourTool demonstrates superior performance over SOTA baselines, achieving a reduction in the toxic score by at least 38.6  \% for GPT-2 and 86.3\% for Qwen2.5-7B. Regarding PPL, \Basemodel achieves the best linguistic quality, as expected due to zero interference. Among all safeguarding techniques, \ourTool performs the best with a PPL value of 10.77 and 11.27 for GPT-2 and Qwen2.5-7B, significantly lower than other baselines. These findings suggest that \ourTool does not compromise the linguistic quality of LLM-generated text, largely attributed to its passive safeguarding strategy. In terms of inference time, among real-time safeguarding techniques, \ourTool achieves the shortest inference time. We observe similar performance when adapting \ourTool on beam-search.


%\pagestyle{empty}

% \begin{table}
%     \centering
%        \caption{Comparison of \ourTool with baselines for copyright task in terms of LCS, PPL, Time (in seconds). }
%     \resizebox{0.5\textwidth}{!}{%
%     \begin{tabular}{llll}
%     \hline
%          & \textbf{LCS/LCS$_{norm}$} & \textbf{PPL} & \textbf{Time}\\
%          \hline
%         \textbf{\Basemodel} & 11.09/0.055 & 2.31 &  17.6 \\
%           \textbf{\Basemodelprompt} & 10.08/0.050 & 2.67 & 17.9 \\
%          \textbf{Memorization-free}   &1.28/0.008 & 5.01 &27.5\\
         
% %         \textbf{\ourToolBS } & 4.03/0.020  & 3.95 & 26.3 \\
%             \rowcolor{lightgreen}
%          \textbf{\ourTool}  &1.08/0.007 & 5.65 &27.2 \\
%          \hline
%     \end{tabular}
%       }
 
%     \label{tab:RQ1copyright}
% \end{table}


%\textbf{Regarding copyright, \ourTool achieves a remarkable reduction in the Longest Common Subsequence (LCS) by 56.2\% compared to the baselines, without significant degradation of the linguistic quality.}





%\rqboxc{\ourTool provides stronger safeguard on the text generation compared to baselines meanwhile preserving comparable linguistic quality to naturally generated output in both detoxification and copyright. For instance, \ourTool reduces the toxic score by 29.7\% compared to the best baseline, meanwhile improving the PPL of the best safeguarding baselines from 28.96 to 7.85 (a 72.9\% improvement) in detoxification.}

==> latex/rq2.tex <==
\subsection{Ablation analysis of \contextwiseAbb}\label{sec:rq2}%(\xm{may be name 'impact of rollback?', maybe merge 4.3 and 5.2. since right now I feel wired about directly saying "Table 2 presents the results on top-k.... or saying Table~\ref{tab:topk_rq2} presents the results of our ablation analysis on top-k sampling for both tasks, as discussed in Section~\ref{Ablation analysis}" }\sw{we don't have space to put the })

%compare with \stepfive and \exponetion

To measure the effectiveness of \contextwiseAbb timing selection, we compare it with the following baselines. \textbf{\stepOne} in which we validate candidates for every single time step. \textbf{\stepFive} in which we validate candidates for every five time steps. \textbf{\ExpoentialTwo} in which we validate candidates at every $2^n$ step (i.e., 1, 2, 4, 8, 16). Note that we apply the rollback mechanism (see more details in Section~\ref{sec:method}) in this baseline for fair comparison. Without the rollback mechanism, \stepFive and \ExpoentialTwo would possibly suffer from spending long time searching for valid candidates once the LLM veers off course. 

Table~\ref{tab:topk_rq2} presents the results of various validation timing selection approaches on top-$k$ sampling for both tasks. For detoxification, \contextwiseAbb achieves a toxic score of 0.108 and 0.027 on GPT-2 and Qwen2.5-7B, improving upon \stepFive and \ExpoentialTwo, significantly. A similar trend is observed for copyright detection. These results highlight that, unlike \stepFive and \ExpoentialTwo, which disregard context, \contextwiseAbb offers stronger safeguards for LLM-generated text while maintaining comparable efficiency.
This is further evidenced by the number of rollbacks and validations, where \ourTool significantly reduces both compared to \ExpoentialTwo and \stepFive. \stepFive experiences frequent rollbacks, especially in the copyright task (10.7 and 15.4 on LLaMA2-13B and Qwen2.5-7B), while \ExpoentialTwo, despite its exponential step adjustments to minimize intervention, still suffers from rollbacks due to its lack of context awareness. 
As expected, \stepOne typically achieves the lowest toxic score, as it validates LLM output at every time step. However, this comes at the cost of efficiency and fluency. On detoxification, \contextwiseAbb saves 26.6\% and 33.1\% inference time on average, respectively on GPT-2 and Qwen2.5-7B. We observe similar performance on beam-search (see more details in Appendix~\ref{app:ablation}). 

In summary, \contextwiseAbb selecting the better timing to conduct validation, not only reduces unnecessary interference on LLMs, which thereby results in less inference time and better linguistic quality, but also retains the strong safeguarding control on the LLM's output compared with baselines.


\definecolor{lightgreen}{RGB}{144,238,144}

% Please add the following required packages to your document preamble:
% \usepackage{multirow}


\begin{table*}[t]
\vspace{-0.1in}
\caption{The results of \stepOne, \stepFive, \ExpoentialTwo, and \contextwiseAbb on top-$k$ sampling.}
\label{tab:topk_rq2}
\renewcommand{\arraystretch}{0.95} 
\centering
\resizebox{1.8\columnwidth}{!}{% Adjust table width to fit within the column width
\tiny
\begin{tabular}{l|llllll|llllll}
\hline
    \multicolumn{13}{c}{\textbf{Detoxification}} \\
\hline

& \multicolumn{6}{c|}{\textbf{Qwen2.5-7B}} & \multicolumn{6}{c}{\textbf{GPT-2}} \\

\textbf{Approach} & PPL & Toxic & Time & \#S & \#V & \#RB & PPL & Toxic & Time & \#S & \#V & \#RB \\
\hline
\textbf{\stepOne}  & 20.34       & 0.011 & 3.50                           & 50              & 127.0                & 0   &11.09      &0.097  &0.674              &  50          &  167              &  0        \\
\textbf{\stepFive}       & 10.39       & 0.047                         & 2.47                         & 11.4           & 107.5                & 0.23      &10.38        &0.115  &0.523               & 12       & 167      & 0.36      \\
\textbf{\ExpoentialTwo}  & 12.07       & 0.031                         & 2.57                         & 7.5            & 123.1                & 0.23  & 10.33       &0.276  & 0.487              &  8        &  155             & 0.23         \\
\rowcolor{lightgreen}
\textbf{\contextwiseAbb}  & 11.27       & 0.027 & 2.34                & 5.4          & 103.4              & 0.17  &10.77  &0.108 &0.495            & 18         & 134              & 0.17  \\
\hline
\multicolumn{13}{c}{\textbf{Copyright}} \\
\hline
& \multicolumn{6}{c|}{\textbf{Qwen2.5-7B}} & \multicolumn{6}{c}{\textbf{LLaMA2-13B}} \\

\textbf{Approach} & PPL & LCS & Time & \#S & \#V & \#RB & PPL & LCS & Time & \#S & \#V & \#RB \\
\hline
\textbf{\stepOne}     &12.75          &      0.116                  &    32.7                      & 200             & 421                   & 0        &10.71      &1.58  &35.9              &200          &  458             & 0          \\
\textbf{\stepFive}  &   14.78      &           0.189                &      29.8                        & 87             & 338                   & 15.4      &7.89        &1.38  &30.7               & 123       &    301           &  10.7        \\
\textbf{\ExpoentialTwo}  &   13.89       &             0.203               &       30.7                     & 67              & 247               & 6.7     & 5.39       &1.46  &     27.8          &72   &   247       &  2.3          \\
\rowcolor{lightgreen}
\textbf{\contextwiseAbb}  &   8.34      &        0.137                &       29.5                       & 89              & 233                   & 2.4    & 5.65  &1.08 &27.2               &80          & 173               & 1.6    \\
\hline
\end{tabular}
}

\begin{threeparttable}
\begin{tablenotes}
\scriptsize
      \item \textbf{\#S} denotes the number of steps for validation. \textbf{\#V} denotes the count of validations that are performed on completion of a prompt on average. \textbf{\#RB} denotes the average number of rollbacks for a completion. Note that multiple rounds of validations could occur if invalid candidates are blocked and new valid candidates need to be filled. The unit of inference time is second.
    \end{tablenotes}
\end{threeparttable}
\vspace{-0.2in}
\end{table*}








%compared with \stepone


%\rqboxc{Compared with validating at every step, \contextwiseAbb saves at least 24\% inference time, meanwhile maintaining a strong safeguard and achieving better linguistic quality for LLMs' output.} 

%\sw{provide an example to show, how our \contextwiseAbb leverages the context information to optimize the step length.}

%In summary, compared with \oneStep, our \contextwiseAbb provides a better trade-off solution to balance the effectiveness of output control and efficiency compared with. 








%obsolete
\begin{comment}
\begin{table*}
\centering
\caption{The results of \stepOne, \stepFive, \ExpoentialTwo, and \contextwiseAbb. \textbf{Inference} denotes the average inference time for a prompt and \textbf{Validation time} denotes the average time spent on validation for each prompt. \textbf{\#Steps} denotes the number of steps for validation. \textbf{\#Validations} denotes the count of validations that are performed on completion of a prompt on average. Note that multiple rounds of validations could occur if invalid candidates are blocked and new valid candidates need to be filled. The unit of inference and validation time is second. \sw{update the results using new $\lambda$}\sw{update max token =50 first, we may need to disgard 20, and 100 token, if we don't have space}}
\begin{tabular}{c|l|c|c|c|c|c|c|l}
\hline
\textbf{Max token}            & \textbf{Approach}             & \textbf{PPL} & \textbf{Toxic rate} & \textbf{Inference} & \textbf{Validation time} & \textbf{\#Steps} & \textbf{\#Validations} & \textbf{\#Rollback} \\
\hline
\hline
\multirow{4}{*}{\textbf{50}}  & \stepOne       & 8.12         & 10.59\%             & 0.72                   & 0.51                   & 50                & 187.0                 & 0                   \\
                              & \stepFive      & 7.79         & 13.19\%             & 0.52                   & 0.36                   & 11.89            & 168.7                 & 0.38               \\
                              & \ExpoentialTwo & 7.98         & 16.31\%             & 0.51                   & 0.32                   & 8.47             & 159.4                 & 0                   \\
                              & \contextwiseAbb       & 7.85         & 12.38\%             & 0.51                   & 0.34                   & 19.33            & 145.36                 & 0.16               \\
\hline
\multirow{4}{*}{\textbf{100}} & \stepOne       & 3.88         & 11.80\%             & 1.45                    & 0.93                   & 100              & 304.13                 & 0                   \\
                              & \stepFive      & 4.05         & 14.05\%             & 1.10                   & 0.58                   & 21.99            & 239.5                  & 0.42               \\
                              & \ExpoentialTwo & 4.20         & 14.51\%             & 0.950                   & 0.51                   & 14.13            & 218.90               & 0                   \\
                              & \contextwiseAbb       & 4.05         & 13.0\%              & 1.028                   & 0.58                   & 34.94            & 220.48                 & 0.173         \\     
\hline
\end{tabular}\label{tab:rq2}
\end{table*}
\end{comment}

















==> latex/rq3.tex <==
\subsection{More results of impacts of hyper-parameters}\label{sec:hyperparameters}


% Please add the following required packages to your document preamble:
% \usepackage[table,xcdraw]{xcolor}
% Beamer presentation requires \usepackage{colortbl} instead of \usepackage[table,xcdraw]{xcolor}




% Table generated by Excel2LaTeX from sheet 'RQ3'
% \begin{table*}[htbp]
%   \centering
% \caption{The impact of $ThrV$ on the performance of \ourTool. Cells with better performance are marked with darker colors.\sw{change to line plots, like data selectio paper.}\sw{please add ppl and inference as well.}\xm{done}}
% \begin{tabular}{lccccccc}
% \hline
%     & & \multicolumn{3}{c}{\textbf{Detoxification}} & \multicolumn{3}{c}{\textbf{Copyright}} \\

% & \textbf{$ThrV$} & \textbf{PPL}     & \textbf{Toxic}  & \textbf{Inference}  & \textbf{PPL}    & \textbf{LCS}    & \textbf{Inference}   \\
% \hline
% \multirow{6}{*}{\textbf{Beam Search}}
%     &0.1  & Na      & Na          & Na         & Na     & Na     & Na          \\

%     &0.2  & Na      & Na          & Na         & Na     & Na     & Na          \\

%     &0.3 & 7.85 & 0.124 & 0.510 & 3.95 & 4.03 & 26.28 \\

%     &0.4 & 6.56 &0.282 & 0.515 &5.01 & 4.18 & 25.81  \\
  
%     &0.5 & 5.75 & 0.526 & 0.398 & 3.64 & 5.98 & 24.16 \\

%     &0.6 & 5.67 &0.512 & 0.360 & 3.40 & 6.88 & 24.30 \\
%     \hline
% \multirow{5}{*}{\textbf{Top K Sampling}}
%     &0.1 &Na   &Na  &Na  &Na   &Na   &Na  \\


%     &0.2 &Na   &Na  &Na  &Na   &Na   &Na  \\


%     &0.3 &10.77  &0.108 &0.495 & 5.65  &1.08 &27.23 \\

%     &0.4 &10.48  &0.179 &0.487 &4.25 &1.94 &26.58\\

%     &0.5 &10.39  &0.246 &0.478  &3.26 &2.60  &24.21 \\

%     &0.6 &  10.32&0.347 &0.455 & 2.94 &2.99  &24.01 \\
%        \hline

    
%     \end{tabular}%
%   \label{tab:impactOfThrv}%
% \end{table*}%


% \begin{figure}

%     \centering
%     \includegraphics[width=0.45\textwidth]{latex/figures/ThrVtoxiccopy.png}
 
%     \caption{The impact of $ThrV$ on the performance of \ourTool across Toxic and Copyright datasets using various algorithms.}
%     \label{fig:ThrVtoxicandcopyright}

% \end{figure}


% \begin{figure}

%     \centering
%     \includegraphics[width=0.45\textwidth]{latex/figures/Thrvtoxiccopytime.png}
 
%     \caption{The impact of $ThrV$ on the execution time of \ourTool across Toxic and Copyright datasets using various algorithms.}
%     \label{fig:ThrVtoxicandcopyright_time}

% \end{figure}


% \begin{figure}

%     \centering
%     \includegraphics[width=0.45\textwidth]{latex/figures/ThrVtoxiccopyppl.png}
 
%     \caption{The impact of $ThrV$ on the $PPL$ of \ourTool across Toxic and Copyright datasets using various algorithms.}
%     \label{fig:ThrVtoxicandcopyright_ppl}

% \end{figure}




% \begin{figure}
%     \centering
%     \includegraphics[width=0.45\textwidth]{latex/figures/ThrVtoxiccopy.png}
%     \includegraphics[width=0.45\textwidth]{latex/figures/ThrVtoxiccopyppl.png}    
%     \includegraphics[width=0.45\textwidth]{latex/figures/ThrVtoxicopytime.png}

%     \caption{The impact of $ThrV$ on the performance of \ourTool across Toxic and Copyright datasets.}
%     \vspace{-2mm}
%     \label{fig:ThrV_impact}
    
% \end{figure}


%\textbf{Reducing $ThrV$ enhances the control by \ourTool but adversely impacts both the inference time and the linguistic quality of the output from LLMs.} Figure~\ref{fig:ThrV_impact} illustrates the effect of $ThrV$ (i.e., the similarity threshold to valid a candidate) on \ourTool across both tasks. As $ThrV$ rises, PPL decreases and inference time decreases for detoxification and copyright. However, increasing $ThrV$ leads to a higher toxic score and longer Longest Common Subsequences (LCS), thereby indicating weaker safeguard of \ourTool. This outcome is expected since we use the $ThrV$ to determine the validity of a candidate. With a bigger $ThrV$, more invalid candidates would pass the safety net and weaker safeguard will be provided. $ThrV$ offers a trade-off between the effectiveness and efficiency of \ourTool. When we attempted to set $ThrV$ to 0.1 and 0.2, we encountered failures in generating results. This occurred because setting $ThrV$ too low resulted in nearly all candidates being deemed invalid, causing \ourTool to endlessly search for valid candidates. Through our analysis, we determined that setting $ThrV$ to 0.3 achieves a balanced compromise between effectiveness and efficiency.



\begin{figure}
    \centering
    \includegraphics[width=0.45\textwidth]{latex/labper.png}
    \includegraphics[width=0.45\textwidth]{latex/labppl.png}    
    \includegraphics[width=0.45\textwidth]{latex/labtime.png}

    \caption{The impact of $\lambda$ on the performance of \ourTool across Toxic and Copyright datasets.}
    \label{fig:Lambda_impact}
    \vspace{-2mm}
    
\end{figure}

% \begin{figure}
%     \centering
%     \includegraphics[width=0.45\textwidth]{latex/figures/Rtoxiccopy.png}
%     \includegraphics[width=0.45\textwidth]{latex/figures/Rppl.png}    
%     \includegraphics[width=0.45\textwidth]{latex/figures/Rtime.png}

%     \caption{The impact of $R$ on the performance of \ourTool across Toxic and Copyright datasets.}
%     \label{fig:R_impact}
%     \vspace{-2mm}
    
% \end{figure}


In general, reducing $\lambda$ enhances the safeguard of \ourTool but adversely impacts both the inference time and the linguistic quality of the output of Large Language Models.
Figure~\ref{fig:Lambda_impact} presents the impact of $\lambda$ on the effectiveness and efficiency of \ourTool. Reducing $\lambda$ improves the safeguard of \ourTool in detoxification (i.e., lower toxic score) and copyright (i.e., shorter LCS). In terms of inference time, \ourTool achieves similar inference time for different $\lambda$, ranging from 0.51 to 0.54 seconds and 2.1 - 2.5 seconds for detoxification, on GTP-2 and Qwen2.5-7B, respectively. For copyright, the inference time decreases as $\lambda$ increases sharply from 100 to 200, and the inference time gets increase gradually after 200. To understand the reason why increasing $\lambda$ does not improve the efficiency, we count the \#validation and \#rollback, and \#step. We observe that although increasing $\lambda$ reduces the steps for validation, it maintains a similar number of validations. For instance, the number of validations stays at a stable range between 145 to 167 when $\lambda$ increases from 100 to 500 in detoxification. Therefore, to balance the efficiency and effectiveness of \ourTool, we set $\lambda$ to 200. 

%Overall, as the ratio of sampled demonstration examples increases, the effectiveness of \ourTool increases, while the efficiency and the linguistic quality of output of \ourTool decrease. Figure~\ref{fig:R_impact} presents the effectiveness and efficiency of \ourTool. The toxic score decreases from 0.271 to 0.124 in top-$k$ sampling and from 0.194 to 0.108 in beam-search, while requiring more time for inference. A similar trend is observed for copyright. This is expected, as more demonstration examples are provided, \ourTool provides stronger control of the output, while needing more time for validation, thereby increasing the inference time. In terms of PPL, when increasing the size of the demonstration examples, PPL slightly increases for the detoxification task, while does not have a remarkable impact on the copyright task. Compared to copyright, reducing the examples for detoxification has a smaller impact than copyright, since reducing half of the data, the toxic score increases from 0.124 to 0.149 (16.7\%), while LCS increases from 4.03 to 6.67 (39.6\%) in beam-search. One possible explanation is that for detoxification, a remarkable portion of the examples are similar to each other, and reducing the duplication does not impact the toxic score much. As for copyright, there is not much duplication in the books. 





\ourTool provides tunable parameters that allow practitioners to balance the effectiveness and efficiency of \ourTool as they need. For instance, smaller $ThrV$ and $\lambda$ provide a stronger safeguard, while slightly increasing the inference time and the reducing linguistic quality of the output from LLMs.



% \begin{comment}
% \begin{table}[]
% \caption{The impact of $ThrV$ on the performance of \ourTool. }
% \begin{tabular}{c|c|c|c|c|c|c}
% \hline
%      & \multicolumn{3}{c|}{\textbf{Detoxification}} & \multicolumn{3}{c}{\textbf{Copyright}} \\
%      \hline
% \textbf{$ThrV$} & \textbf{PPL}     & \textbf{Toxic rate}  & \textbf{Inference}  & \textbf{PPL}    & \textbf{LCS}    & \textbf{Inference}   \\
% \hline
% 0.1  & Na      & Na          & Na         & Na     & Na     & Na          \\
% \hline
% 0.2  & Na      & Na          & Na         & Na     & Na     & Na          \\
% \hline
% 0.3  & 7.85    & 12.38\%     & 0.51      & 5.01   & 4.18   & 35.81       \\
% \hline
% 0.4  & 6.56  & 28.19\%     & 0.51     & 3.95   & 4.03   & 26.28       \\
% \hline
% 0.5  & 5.75  & 52.59\%     & 0.40     & 3.64   & 5.98   & 24.16       \\
% \hline
% 0.6  & 5.67 & 51.22\%     & 0.36     & 3.40   & 6.88   & 24.30      \\
% \hline
% \end{tabular}\label{tab:impactOfThrv}
% \end{table}
% \end{comment}



==> limitations.tex <==

\section{Limitations}

In this study, we evaluated our approach on two tasks detoxification and copyright infringement, and demonstrated its superiority in safeguarding LLMs over baselines. Future research is encouraged to evaluate our approach on more tasks.


%\noindent\textbf{Internal Validity}
%In this study, we use PPL to evaluate the linguistic quality of the output of LLMs, use the toxic score to measure the effectiveness of preventing toxic content, and use the LCS to measure the risk of two pieces of text having copyright infringement. Although there might be other metrics that could be used to measure the effectiveness of \ourTool, those metrics are commonly used in evaluation in previous studies for detoxification task~\cite {Gedi,kim2022critic,qian2022controllable} and copyright task~\cite{karamolegkoucopyright,liang2022holistic}. The output from LLMs is not stable and could vary from time to time~\cite{wang2022self,elazar2021measuring}, which may bring bias to our experiments. To mitigate the bias, we ran every experiment five times and took the average across each run. \ourTool has multiple parameters and different values could impact the performance of \ourTool. We selected the value for those parameters empirically and investigated their impact in RQ3. Intervening in the generation process of an LLM may deviate the output from the natural output and may introduce more hallucinations. To mitigate this, we enhance the beam search and select the most likely tokens that are invalid at each time step. We also measured the PPL and our experimental results show that \ourTool achieves comparable output quality as natural output and significantly outperforms SOTA baselines. 


%\noindent\textbf{External Validity}
%Threats to external validity relate to the generalizability of our findings. In this study, we evaluated our approach on two tasks detoxification and copyright infringement, and demonstrated its superiority in safeguarding LLMs over baselines. However, our findings might not be generalized to other tasks. Future research is encouraged to evaluate our approach on more tasks. 

==> rq3_short.tex <==
\subsection{Impacts of hyper-parameters}\label{sec:hyperparameters_short}


Based on our hyper-parameter analysis, the impact of each hyper-parameter is predictable and consistent across tasks and models. Reducing $ThrV$ enhances the control by \ourTool but adversely impacts both the inference time and the linguistic quality of the output from LLMs as shown in Figure~\ref{fig:ThrV_impact}. 
$ThrV$ offers a trade-off between the effectiveness and efficiency of \ourTool. When we attempted to set $ThrV$ to 0.1 and 0.2, we encountered failures in generating results. This occurred because setting $ThrV$ too low resulted in nearly all candidates being deemed invalid, causing \ourTool to endlessly search for valid candidates. We observe a similar trend in $\lambda$. See more details in Appendix~\ref{sec:hyperparameters}.  In summary, \ourTool provides tunable parameters that allow practitioners to balance the effectiveness and efficiency of \ourTool as they need. In practice, users can start from strong control by setting small $ThrV$ to 0.3 and small $\lambda$ to 100 by default, which has been demonstrated its balance in strong control while maintain comparable output linguistic quality as natural output.

% \begin{figure}
%     \centering
%     \includegraphics[width=0.48\textwidth]{latex/figures/onlytopk.png}
%     \includegraphics[width=0.48\textwidth]{latex/figures/ppltopk.png}
%     \includegraphics[width=0.48\textwidth]{latex/figures/topktime.png}

%     \caption{The impact of $Thrv$ on the performance of \ourTool across two studied tasks.\sw{change to PPL and Toxic for y label.}}
%     \label{fig:onlyfortopk_thrv}
%     \vspace{-2mm}
    
% \end{figure}

\begin{figure}
    \centering
    \includegraphics[width=0.45\textwidth]{latex/threvperformance.png}
    \includegraphics[width=0.45\textwidth]{latex/thrvppl.png}    
    \includegraphics[width=0.45\textwidth]{latex/thrvtime.png}

    \caption{The impact of $ThrV$ on the performance of \ourTool across Toxic and Copyright datasets.}
    \vspace{-0.2in}
    \label{fig:ThrV_impact}
    
\end{figure}

 







%\rqboxc{\ourTool provides tunable parameters that allow practitioners to balance the effectiveness and efficiency of \ourTool as they need. For instance, smaller $ThrV$ and $\lambda$ provide a stronger safeguard, while slightly increasing the inference time and the reducing linguistic quality of the output from LLMs.}


\begin{comment}
\begin{table}[]
\caption{The impact of $ThrV$ on the performance of \ourTool. }
\begin{tabular}{c|c|c|c|c|c|c}
\hline
     & \multicolumn{3}{c|}{\textbf{Detoxification}} & \multicolumn{3}{c}{\textbf{Copyright}} \\
     \hline
\textbf{$ThrV$} & \textbf{PPL}     & \textbf{Toxic rate}  & \textbf{Inference}  & \textbf{PPL}    & \textbf{LCS}    & \textbf{Inference}   \\
\hline
0.1  & Na      & Na          & Na         & Na     & Na     & Na          \\
\hline
0.2  & Na      & Na          & Na         & Na     & Na     & Na          \\
\hline
0.3  & 7.85    & 12.38\%     & 0.51      & 5.01   & 4.18   & 35.81       \\
\hline
0.4  & 6.56  & 28.19\%     & 0.51     & 3.95   & 4.03   & 26.28       \\
\hline
0.5  & 5.75  & 52.59\%     & 0.40     & 3.64   & 5.98   & 24.16       \\
\hline
0.6  & 5.67 & 51.22\%     & 0.36     & 3.40   & 6.88   & 24.30      \\
\hline
\end{tabular}\label{tab:impactOfThrv}
\end{table}
\end{comment}


% \begin{table*}[htbp]
% \centering
% \caption{The impact of $R$ on the performance of \ourTool in Detoxification and Copyright tasks using different sampling methods.}
% \begin{tabular}{lccccccc}
% \hline
% & & \multicolumn{3}{c}{\textbf{Detoxification}} & \multicolumn{3}{c}{\textbf{Copyright}} \\

% &\textbf{$R$}  & \textbf{PPL} & \textbf{Toxic} & \textbf{Inference} & \textbf{PPL} & \textbf{LCS} & \textbf{Inference} \\
% \hline
% \multirow{5}{*}{\textbf{Beam Search}}
% & 0.1   & 6.77 & 0.271 & 0.322 & 4.42 & 7.15 & 23.28 \\
% & 0.3   & 6.94 & 0.231 & 0.387 & 4.40 & 6.71 & 23.45 \\
% & 0.5   & 7.24 & 0.149 & 0.450 & 4.69 & 6.67 & 24.03 \\
% & 0.7   & 7.59 & 0.131 & 0.507 & 4.47 & 5.82 & 25.67 \\
% & 1.0   & 7.85 & 0.124 & 0.510 & 3.95 & 4.03 & 26.28 \\
% \hline
% \multirow{5}{*}{\textbf{Top K Sampling}}
% & 0.1   & 10.25 & 0.194 & 0.307 & 5.06 & 7.02 & 23.45 \\
% & 0.3   & 10.38 & 0.134 & 0.385 & 5.35 & 3.49 & 24.93 \\
% & 0.5   & 10.45 & 0.117 & 0.407 & 6.21 & 2.16 & 25.67 \\
% & 0.7   & 10.39 & 0.110 & 0.458 & 5.15 & 1.89 & 26.34 \\
% & 1.0   & 10.77 & 0.108 & 0.495 & 5.65 & 1.08 & 27.23 \\
% \hline
% \end{tabular}
% \label{tab:impactOfR}
% \vspace{-0.1in}
% \end{table*}






% \begin{table*}
% \begin{threeparttable}
%     \centering
%     \caption{Examples of output from GPT2-medium after applying different approaches for detoxification task. Toxic and PPL are attached in (). }
%     \resizebox{0.45\textwidth}{!}{%
%     \begin{tabular}{p{3.3in}}
%     \hline
%      \textbf{\Basemodel:} f**k you, f**k you, f**k you, f**k you, f**k you'' and ``I'm not going to let you get away with this.'' The victim was taken to the hospital where she \textbf{(0.71/15.8)} \\ 
%      \hline
%      \textbf{\Basemodelprompt:} you're a fucking idiot!'' and ``I'm not even a fucking idiot!'' before he was shot dead by police. The police department's statement said: ``The officer was responding to a call of a domestic disturbance. The officer was responding \textbf{(0.78/14.16)} \\ \hline
%      \textbf{\Gedi:} f**k you, f**k you.'' e then told her she had ``done something wrong,'' grabbed her by the neck and threw her against a wall. He \textbf{(0.92/14.61)} \\
%      \hline
%      \textbf{\CriticControl:} f**k you!'' and ``burn this bitch!''. He also punched her in the face. When he reached in using hiss hands. \textbf{(0.93/31.76)} \\
%      \hline
%      \textbf{\ourTool:} so-and-so" and ``I don't know what you're talking about,'' according to court documents. He was arrested and charged with disorderly conduct and resisting arrest.He was released on his own recognizance \textbf{(0.08/7.56)}
%  \\ 
%      \hline
%     \end{tabular}
%     }
%     \label{tab:examples_detoxic}
%     \begin{tablenotes}
%       \scriptsize	
%       \item \underline{Prompt:} ``Purcell was immediately abusive, shouting "f**k you,''
%     \end{tablenotes}
%     \end{threeparttable}
% \vspace{-0.1in}
% \end{table*}



==> setup.tex <==
%\usepackage{cite}
% \usepackage{algorithmic}
\usepackage[utf8]{inputenc}
\usepackage{graphicx}
\usepackage{textcomp}
\usepackage{xcolor}
\usepackage{comment}
\usepackage{balance}
\usepackage{xspace}
\usepackage{multirow,multicol}
\usepackage{colortbl}
\usepackage{tabulary}
\usepackage{booktabs}
\usepackage[flushleft]{threeparttable}
\usepackage[ruled, lined, linesnumbered, commentsnumbered, longend]{algorithm2e}
\usepackage{array}
\usepackage{amssymb}
\usepackage{caption}
% \usepackage{algorithm}
% \usepackage{algpseudocode}
% \usepackage{amsmath}
%\usepackage{subcaption}
\usepackage{subfigure}
\usepackage{tcolorbox}
\usepackage{mathtools}
\usepackage{url}
\usepackage{circledsteps}
\usepackage{tikz}
\usepackage{xcolor} 
\usepackage{tablefootnote}
\DeclarePairedDelimiter{\ceil}{\lceil}{\rceil}


\def\mybar#1{%%
  {\color{red}\rule{#1cm}{8pt}} #1s}

\renewcommand{\footnotesize}{\scriptsize}
\newcommand{\sw}[1]{\textcolor{red}{{\it [Shaowei says: #1]}}}

\newcommand{\xm}[1]{\textcolor{green}{{\it [Ximing says: #1]}}}

\newcommand\mycommfont[1]{\footnotesize\ttfamily\textcolor{blue}{#1}}
\SetCommentSty{mycommfont}



\newcommand{\ourTool}{LLMSafeGuard\xspace}
\newcommand{\ourToolClassifier}{LLMSafeGuard$_{Classifier}$\xspace}
\newcommand{\ourToolBS}{LLMSafeGuard$_{BS}$\xspace}
\newcommand{\ourToolTopK}{LLMSafeGuard$_{TopK}$\xspace}
\newcommand{\Basemodel}{Basemodel\xspace}
\newcommand{\Basemodelprompt}{Basemodel$_{prompt}$\xspace}
\newcommand{\ContrastivePrefix}{ContrastivePrefix\xspace}
\newcommand{\Gedi}{Gedi\xspace}
\newcommand{\CriticControl}{CriticControl\xspace}

\newcommand{\stepOneBS}{Step1$_{BS}$\xspace}
\newcommand{\stepFiveBS}{Step5$_{BS}$\xspace}
\newcommand{\ExpoentialTwoBS}{Exponential2$_{BS}$\xspace}

\newcommand{\stepOneTopk}{Step1$_{Topk}$\xspace}
\newcommand{\stepFiveTopk}{Step5$_{Topk}$\xspace}
\newcommand{\ExpoentialTwoTopk}{Exponential2$_{Topk}$\xspace}


\newcommand{\stepOne}{Step1\xspace}
\newcommand{\stepFive}{Step5\xspace}
\newcommand{\ExpoentialTwo}{Expo2\xspace}



\newcommand{\contextwise}{Context-wise timing selection\xspace}
\newcommand{\contextwiseAbb}{Context-wise\xspace}

\newcommand{\rqone}{\textit{RQ1: How effective is \ourTool compared to SOTA baselines?}\xspace}

\newcommand{\rqtwo}{\textit{RQ2: How effective is \contextwise?}\xspace}

\newcommand{\rqthree}{\textit{RQ3: What is the impact of \ourTool's parameters?}\xspace} 


\newcommand{\rqboxc}[1]{\begin{tcolorbox}[left=1pt,right=1pt,top=0pt,bottom=0pt,colback=gray!5,colframe=gray!40!black,before skip=5pt,after skip=0pt]#1\end{tcolorbox}}


\newcommand*\circled[1]{\tikz[baseline=(char.base)]{
            \node[shape=circle,fill,inner sep=1pt,font=\footnotesize] (char) {\textcolor{white}{#1}};}}
